Backward iteration in strongly convex domains

We prove that a backward orbit with bounded Kobayashi step for a hyperbolic or strongly elliptic holomorphic self-map of a bounded strongly convex domain in the d-dimensional complex Euclidean space necessarily converges to a boundary fixed point, generalizing previous results obtained by Poggi-Corradini in the unit disk and by Ostapyuk in the unit ball.

==> 2417967.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% These are the macroes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifsect\newif\iffinal
\secttrue\finalfalse
\def\thm #1: #2{\medbreak\noindent{\bf #1:}\if(#2\thmp\else\thmn#2\fi}
\def\thmp #1) { (#1)\thmn{}}
\def\thmn#1#2\par{\enspace{\sl #1#2}\par
        \ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\def\square{{\msam\char"03}}
\def\qedn{\thinspace\null\nobreak\hfill\square\par\medbreak}
\def\pf{\ifdim\lastskip<\smallskipamount \removelastskip\smallskip\fi
        \noindent{\sl Proof\/}:\enspace}
\def\itm#1{\item{\rm #1}\ignorespaces}
\let\smbar=\bar
\def\bar#1{\overline{#1}}
%
%\input pdfcolor
%
%\input boxedeps
%\input boxedeps.cfg
%\HideDisplacementBoxes
%%
%\def\Figuraeps #1 (#2){\message{Figura #1}
%	\midinsert      
%	\centerline{\BoxedEPSF{#2.eps}}
%	\bigskip
%	\centerline{\bf Figure~#1}
%	\endinsert}
%%
%\def\Figurascaledeps #1 (#2)(#3){\message{Figura #1}
%	\midinsert      
%	\centerline{\BoxedEPSF{#2.eps scaled #3}}
%	\bigskip
%	\centerline{\bf Figure~#1}
%	\endinsert}
%
%
\newcount\parano
\newcount\eqnumbo
\newcount\thmno
\newcount\versiono
\newcount\remno
\newbox\notaautore
\def\neweqt#1$${\xdef #1{(\number\parano.\number\eqnumbo)}
    \eqno #1$$
    \global \advance \eqnumbo by 1}
\def\newrem #1\par{\global \advance \remno by 1
    \medbreak
{\bf Remark \the\parano.\the\remno:}\enspace #1\par
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\def\newthmt#1 #2: #3{\xdef #2{\number\parano.\number\thmno}
    \global \advance \thmno by 1
    \medbreak\noindent
    {\bf #1 #2:}\if(#3\thmp\else\thmn#3\fi}
\def\neweqf#1$${\xdef #1{(\number\eqnumbo)}
    \eqno #1$$
    \global \advance \eqnumbo by 1}
\def\newthmf#1 #2: #3{\xdef #2{\number\thmno}
    \global \advance \thmno by 1
    \medbreak\noindent
    {\bf #1 #2:}\if(#3\thmp\else\thmn#3\fi}
\def\forclose#1{\hfil\llap{$#1$}\hfilneg}
\def\newforclose#1{
	\ifsect\xdef #1{(\number\parano.\number\eqnumbo)}\else
	\xdef #1{(\number\eqnumbo)}\fi
	\hfil\llap{$#1$}\hfilneg
	\global \advance \eqnumbo by 1
	\iffinal\else\rsimb#1\fi}
\def\forevery#1#2$${\displaylines{\let\eqno=\forclose
        \let\neweq=\newforclose\hfilneg\rlap{$\qquad\quad\forall#1$}\hfil#2\cr}$$}
%
\def\noNota #1\par{}
\def\today{\ifcase\month\or
   January\or February\or March\or April\or May\or June\or July\or August\or
   September\or October\or November\or December\fi
   \space\number\year}
\def\inizia{\ifsect\let\neweq=\neweqt\else\let\neweq=\neweqf\fi
\ifsect\let\newthm=\newthmt\else\let\newthm=\newthmf\fi}
\def\bititolo{\empty}
\gdef\begin #1 #2\par{\xdef\titolo{#2}
\ifsect\let\neweq=\neweqt\else\let\neweq=\neweqf\fi
\ifsect\let\newthm=\newthmt\else\let\newthm=\newthmf\fi
\iffinal\let\Nota=\noNota\fi
\centerline{\titlefont\titolo}
\if\bititolo\empty\else\medskip\centerline{\titlefont\bititolo}
\xdef\titolo{\titolo\ \bititolo}\fi
\bigskip
\centerline{\bigfont
\autore \ifvoid\notaautore\else\footnote{${}^1$}{\unhbox\notaautore}\fi}
\bigskip\if\istituto!\centerline{\today}\else
\centerline{\istituto}
\centerline{\indirizzo}
\centerline{\email}
\medskip
\centerline{#1\ \anno}\fi
\bigskip\bigskip
\ifsect\else\global\thmno=1\global\eqnumbo=1\fi}
\def\anno{2011}
%
\def\raggedleft{\leftskip2cm plus1fill \spaceskip.3333em \xspaceskip.5em
\parindent=0pt\relax}
%\def\dafare{\par\smallskip\begingroup\Bittersweet\raggedleft}
%\def\enddafare{\par\endgroup\pdfsetcolor{0. 0. 0. 1.}\smallbreak}
%\def\danota{\par\begingroup\ForestGreen\raggedleft}
%\let\enddanota=\enddafare
%\def\datogliere{\par\begingroup\Blue\raggedleft}
%\let\enddatogliere=\enddafare
%
\font\titlefont=cmssbx10 scaled \magstep1
\font\bigfont=cmr12
\font\eightrm=cmr8
\font\sc=cmcsc10
\font\bbr=msbm10
\font\sbbr=msbm7
\font\ssbbr=msbm5
\font\msam=msam10
\font\gto=eufm10
\font\bfm=cmmib10
\font\bfsy=cmbsy10
\def\ca #1{{\cal #1}}
\def\gt #1{\hbox{\gto #1}}
\nopagenumbers
\binoppenalty=10000
\relpenalty=10000
\newfam\amsfam
\textfont\amsfam=\bbr \scriptfont\amsfam=\sbbr \scriptscriptfont\amsfam=\ssbbr
\newfam\boldifam
\textfont\boldifam=\bfm
%
\let\de=\partial
\let\eps=\varepsilon
\let\phe=\varphi
\def\Hol{\mathop{\rm Hol}\nolimits}
\def\Aut{\mathop{\rm Aut}\nolimits}
\def\Hom{\mathop{\rm Hom}\nolimits}
\def\Fix{\mathop{\rm Fix}\nolimits}
\def\Sing{\mathop{\rm Sing}\nolimits}
\def\End{\mathop{\rm End}\nolimits}
\def\Ker{\mathop{\rm Ker}\nolimits}
\def\Res{\mathop{\rm Res}\nolimits}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\sp{\mathop{\rm sp}\nolimits}
\def\id{\mathop{\rm id}\nolimits}
\def\rk{\mathop{\rm rk}\nolimits}
\def\ord{\mathop{\rm ord}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\Jac{\mathop{\rm Jac}\nolimits}
\def\Span#1{\mathop{\rm Span}\nolimits\left(#1\right)}
\def\bigoperp{\mathop{\hbox{$\bigcirc\kern-11.8pt\perp$}}\limits}
\def\hz{\hat{z}}
\def\hf{\hat{f}}
\def\hg{\hat{g}}
\def\ha{\hat{a}}
\def\hb{\hat{b}}
\mathchardef\void="083F
\mathchardef\ellb="0960
\mathchardef\taub="091C
\def\C{{\mathchoice{\hbox{\bbr C}}{\hbox{\bbr C}}{\hbox{\sbbr C}}
{\hbox{\sbbr C}}}}
\def\R{{\mathchoice{\hbox{\bbr R}}{\hbox{\bbr R}}{\hbox{\sbbr R}}
{\hbox{\sbbr R}}}}
\def\N{{\mathchoice{\hbox{\bbr N}}{\hbox{\bbr N}}{\hbox{\sbbr N}}
{\hbox{\sbbr N}}}}
\def\P{{\mathchoice{\hbox{\bbr P}}{\hbox{\bbr P}}{\hbox{\sbbr P}}
{\hbox{\sbbr P}}}}
\def\Q{{\mathchoice{\hbox{\bbr Q}}{\hbox{\bbr Q}}{\hbox{\sbbr Q}}
{\hbox{\sbbr Q}}}}
\def\Z{{\mathchoice{\hbox{\bbr Z}}{\hbox{\bbr Z}}{\hbox{\sbbr Z}}
{\hbox{\sbbr Z}}}}
\def\Downarrow{\Big\downarrow}
\def\mapright#1{\smash{\mathop{\longrightarrow}\limits^{#1}}}
\def\rmapdown#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\lmapdown#1{\llap{$\vcenter{\hbox{$\scriptstyle#1$}}$}\Big\downarrow}
\def\arrowbar{\top}
\def\Downmapsto{\vcenter{\offinterlineskip\halign{\hfil$##$\hfil\cr
\arrowbar\cr\Downarrow\cr}}}
%
\newcount\notitle
\notitle=1
\headline={\ifodd\pageno\rhead\else\lhead\fi}
\def\rhead{\ifnum\pageno=\notitle\iffinal\hfill\else\hfill\tt Version
\the\versiono; \the\day/\the\month/\the\year\fi\else\hfill\eightrm\titolo\hfill
\folio\fi}
\def\lhead{\ifnum\pageno=\notitle\hfill\else\eightrm\folio\hfill\autore\hfill
\fi}
%
\newbox\bibliobox
\def\setref #1{\setbox\bibliobox=\hbox{[#1]\enspace}
    \parindent=\wd\bibliobox}
\def\biblap#1{\noindent\hang\rlap{[#1]\enspace}\indent\ignorespaces}
\def\art#1 #2: #3! #4! #5 #6 #7-#8 \par{\biblap{#1}#2: {\sl #3\/}.
    #4 {\bf #5} (#6)\if.#7\else, \hbox{#7--#8}\fi.\par\smallskip}
\def\book#1 #2: #3! #4 \par{\biblap{#1}#2: {\bf #3.} #4.\par\smallskip}
\def\coll#1 #2: #3! #4! #5 \par{\biblap{#1}#2: {\sl #3\/}. In {\bf #4,}
#5.\par\smallskip}
\def\pre#1 #2: #3! #4! #5 \par{\biblap{#1}#2: {\sl #3\/}. #4, #5.\par\smallskip}
%
\def\Bittersweet{\pdfsetcolor{0. 0.75 1. 0.24}} % PANTONE 167
\def\Black{\pdfsetcolor{0. 0. 0. 1.}} % PANTONE 167
\def\raggedleft{\leftskip2cm plus1fill \spaceskip.3333em \xspaceskip.5em
\parindent=0pt\relax}
\def\Nota #1\par{\medbreak\begingroup\Bittersweet\raggedleft
#1\par\endgroup\Black
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
%
\def\ragcn{\leftskip=0pt plus 4em \rightskip=\leftskip
\parfillskip=0pt \spaceskip=0.3333em \xspaceskip=0.5em
\pretolerance=9999 \tolerance=9999 \hyphenpenalty=9999
\exhyphenpenalty=9999}
%
\newcount\defno
\def\smallsect #1. #2\par{\bigbreak\noindent{\bf #1.}\enspace{\bf #2}\par
    \global\parano=#1\global\eqnumbo=1\global\thmno=1\global\defno=0\global\remno=0
    \nobreak\smallskip\nobreak\noindent\message{#2}}
\def\newdef #1\par{\global \advance \defno by 1
    \medbreak
{\bf Definition \the\parano.\the\defno:}\enspace #1\par
\ifdim\lastskip<\medskipamount \removelastskip\penalty 55\medskip\fi}
\finaltrue
\versiono=3
%

\magnification\magstephalf

%%%% Abbreviazioni
\let\no=\noindent
\let\bi=\bigskip
\let\me=\medskip
\let\sm=\smallskip
\let\ce=\centerline
\let\ri=\rightline
\let\te=\textstyle
\let\gd=\goodbreak
\let\io=\infty
\def\mlog{\mathop{{\te{1\over2}\log}}}
\def\qqquad{\quad\qquad}

%
\def\autore{Marco Abate${}^1$\footnote{}{\eightrm 2010 Mathematics Subject Classification: Primary 32H50, 37F99}, Jasmin Raissy${}^2$\footnote{${}^*$}{\eightrm Partially supported by FSE, Regione Lombardia.}}
\def\indirizzo{\vbox{\hfill${}^2$Dipartimento di Matematica e Applicazioni, Universit\`a
di Milano Bicocca,\hfill\break\null\hfill Via Cozzi 53, 20125 Milano, Italy.
E-mail: jasmin.raissy@unimib.it\hfill\null}}
\def\istituto{\vbox{\hfill${}^1$Dipartimento di Matematica, Universit\`a
di Pisa,\hfill\break\null\hfill Largo Pontecorvo 5, 56127 Pisa,
Italy. E-mail: abate@dm.unipi.it\hfill\null\vskip5pt}}
\def\email{}%{\vbox{\hfill${}^2$Kansas State University, 138 Cardwell Hall, Manhattan, KS66505, USA\hfill\break\null\hfill E-mail: ostapyuk@math.ksu.edu\hfill\null\vskip5pt}}
%
%\footnote{}{\eightrm $^*$ Partially supported by FSE, Regione Lombardia.}

\begin {April} Backward iteration in strongly convex domains

{{\narrower{\sc Abstract.}  We prove that a backward orbit with bounded Kobayashi step for a hyperbolic, parabolic or strongly elliptic holomorphic self-map of a bounded strongly convex $C^2$ domain in $\C^d$ necessarily converges to a repelling or parabolic boundary fixed
point, generalizing previous results obtained by Poggi-Corradini in the unit disk and by
Ostapyuk in the unit ball of~$\C^d$. \par
}}
\smallsect 0. Introduction

The theory of non-invertible discrete dynamical systems (that is, the iteration theory of a non-invertible self-map~$f\colon X\to X$ of a set $X$) 
is usually devoted to the study of the behavior of forward orbits of the system (that is, of
sequences of the form $\{f^n(x)\}_{n\in\N}$, where $x\in X$ and $f^n$ denotes the composition of $f$ with
itself $n$ times). In this paper we shall instead study the behavior of {\sl backward orbits,} that is of sequences $\{x_n\}_{n\in\N}$ such that $f(x_{n+1})=x_n$ for all $n\in\N$, in the context of
holomorphic self-maps of bounded strongly convex domains.
\def\autore{Marco Abate %, Olena Ostapyuk 
and Jasmin Raissy}

Backward orbits (also called {\sl backward iteration sequences\/}) for
holomorphic self-maps of the unit disk $\Delta\subset\C$ have been studied by
Poggi-Corradini in [PC2]. He proved that (unless $f$ is a non-Euclidean rotation of~$\Delta$) a backward orbit must converge to a point in the boundary of~$\Delta$, which is (in the sense
of non-tangential limits) a repelling or parabolic
fixed point of the map~$f$. Ostapyuk [O] generalized Poggi-Corradini's
results to backward orbits in the unit ball $B^d\subset\C^d$. The aim of this paper is to
extend Poggi-Corradini's results to backward orbits in general bounded strongly convex
$C^2$ domains in~$\C^n$. To do so, we shall systematically use the geometric
properties of the Kobayashi distance of strongly convex domains; and it is interesting to
notice that the better geometric understanding given by this tool (and the impossibility of
using the kind of explicit computations done in [O] for the ball) yields proofs that are both simpler
and clearer than the previous ones, even for the ball and the unit disk.

To state precisely, and put in the right context, our results, let us first describe 
what is known about holomorphic discrete dynamical systems in strongly
convex domain. As proved several years ago by one of us (see [A1, 2, 3]), the fundamental dychotomy for holomorphic dynamics in complex taut manifolds
is between self-maps whose sequence of iterates is compactly divergent and self-maps 
whose sequence of iterates is relatively compact in the space of all holomorphic self-maps
of the manifold (endowed with the compact-open topology, which is equivalent to the topology
of pointwise convergence). In a convex domain $D$, it turns out that the sequence of iterates of
a holomorphic self-map $f\in\Hol(D,D)$ is compactly divergent if and only if $f$ has no
fixed points inside~$D$; so the dychotomy is between self-maps without fixed points and maps
with fixed points.

Following the usual one-variable terminology, we shall call {\sl elliptic} 
a holomorphic self-map of a bounded convex domain~$D\subset\C^n$ with a not empty fixed point set. If $f\in\Hol(D,D)$
is elliptic, then the dynamics of $f$ is concentrated along a, possibly lower-dimensional, 
convex domain $D_0$, the {\sl limit manifold} of $f$,
in the sense that all limits of subsequences of iterates of~$f$ are given by the composition
of a holomorphic retraction of~$D$ onto $D_0$ with an automorphism of~$D_0$. 
Clearly, $D_0$ contains the fixed point set of~$f$, but in general can be strictly larger;
furthermore, $f|_{D_0}$ is an automorphism of~$D_0$, generating a group whose closure
is the product of a torus with a finite cyclic group (see [A3]). In particular,
backward orbits in~$D_0$ are just forward orbits for the inverse of $f|_{D_0}$, and so their 
behavior is known; for this reason here we shall instead study backward orbits for maps, called {\sl strongly elliptic\/},
whose limit manifold reduces to a point, necessarily fixed. In particular, $f$ is strongly elliptic if and only if the sequence
of iterates of any $x\in D$ converges to a point $p\in D$, which is thus an {\sl attracting} fixed point.

When $f\in\Hol(D,D)$ has no fixed points, and $D\subset\C^d$ is a bounded strongly convex $C^2$ domain, the main dynamical fact is the generalization [A1] of the classical Wolff-Denjoy theorem,
saying that the sequence of iterates converges to a point $\tau\in\de D$, the {\sl Wolff point}
of~$f$. The Wolff point is a {\sl boundary fixed point,} in the sense that
$f$ has $K$-limit~$\tau$ at~$\tau$ (see Section~1 for the precise definition of {\sl $K$-limit,}
also known as {\sl admissible limit;} here it just suffices to say that the existence of the $K$-limit
implies the existence of the non-tangential limit, and thus our $f$ has non-tangential limit~$\tau$
at~$\tau$). Furthermore, it is possible to define the {\sl boundary dilation}~$\beta_\tau$ at~$\tau$, which,
roughly speaking, is the derivative of the normal component of~$f$ along the normal direction
to~$\de D$ at~$\tau$ (and is the natural generalization of the one-variable angular derivative);
and the fact that forward orbits converge to~$\tau$ implies that $0<\beta_\tau\le 1$. Again following the classical one-variable
terminology, we shall say that $f$ is {\sl hyperbolic} and $\tau$ is {\sl attracting} if $0<\beta_\tau<1$; and that $f$ and $\tau$ are
{\sl parabolic} if $\beta_\tau=1$.

Before turning our attention to backward orbits, a final remark is needed. Forward orbits always have {\sl bounded Kobayashi step,} that is the Kobayashi distance $k_D\bigl(f^{n+1}(z),f^n(z)\bigr)$
between two consecutive elements of the orbit is bounded by a constant independent of~$n$ (but depending on the orbit): indeed, $k_D\bigl(f^{n+1}(z),f^n(z)\bigr)\le k_D\bigl(f(z),z\bigr)$, because the Kobayashi
distance~$k_D$ is weakly contracted by holomorphic maps. 
  
Summing up, if $f\in\Hol(D,D)$ is strongly elliptic, hyperbolic or parabolic, then all forward
orbits (have bounded Kobayashi step and) converge to the Wolff point $\tau\in\bar{D}$
(for the sake of uniformity, we are calling {\sl Wolff point} the unique fixed point of 
a strongly elliptic map too), which
is an attracting or parabolic (possibly boundary) fixed point. 
Our main result states that, analogously, backward orbits with bounded Kobayashi step 
for a strongly elliptic, hyperbolic or parabolic map always converge to a repelling or parabolic
boundary fixed point, where a {\sl boundary fixed point} is a point $\sigma\in\de D$ such that
$f$ has $K$-limit $\sigma$ at~$\sigma$, and $\sigma$ is {\sl repellng} if the boundary dilation~$\beta_\sigma$ of~$f$ at~$\sigma$ is larger than~1. 

More precisely, in Section~2 we shall prove the following 

\newthm 
Theorem \OJMz:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be either hyperbolic, parabolic, or strongly elliptic, with Wolff point $\tau\in\bar{D}$. 
Let $\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step.
Then:
\smallskip
\item{\rm (i)} the sequence $\{z_n\}$ converges to a repelling or parabolic 
boundary fixed point~$\sigma\in\de D$;
\itm{(ii)} if $f$ is strongly elliptic or hyperbolic then $\sigma$ is repelling;
\item{\rm (iii)} if $\sigma = \tau$, then $f$ is parabolic;
\item{\rm (iv)} $\{z_n\}$ goes to~$\sigma$ inside a $K$-region, that is, 
there exists $M>0$ so that $z_n\in K_{p}(\sigma,M)$ eventually,\break\indent where $p$ is any point in $D$. 

See Section~1 for (preliminaries and in particular) the definition of $K$-region; going to the boundary inside a $K$-region is
the natural several variables generalization of the one-variable notion of non-tangential approach.

To show that our theorem is not empty we must prove the existence of backward orbits with bounded Kobayashi step. This is done 
in Section~3 where, slightly adapting an argument due to Poggi-Corradini ([PC1]; see also [O]),
we shall prove that if $\sigma\in\de D\setminus\{\tau\}$ is an isolated 
repelling boundary point for $f\in\Hol(D,D)$ strongly elliptic, hyperbolic or parabolic, then there always exist a backward orbit with bounded Kobayashi
step converging to~$\sigma$. 
 
Finally, we would like to thank Pietro Poggi-Corradini and Olena Ostapyuk for bringing this
problem to our attention, and N\'uria Fagella and the Institut de Matem\`atica, Universitat de Barcelona, for their warm hospitality during the completion of this work.

\smallsect 1. Preliminaries

In this section we shall collect a few facts about the geometry of the Kobayashi distance 
and the dynamics of holomorphic self-maps of bounded strongly convex domains 
needed in the rest of the paper.

Let us briefly recall the definition and the main properties of the Kobayashi distance;
we refer to [A2], [JP] and [K] for details and much more. Let $k_\Delta$ denote the 
Poincar\'e distance on the unit disk~$\Delta\subset\C$. If $X$ is a complex manifold,
the {\sl Lempert function}~$\delta_X\colon X\times X\to\R^+$ of~$X$ is defined by
$$
\delta_X(z,w)=\inf\{k_\Delta(\zeta,\eta)\mid
\hbox{$\exists\phi\colon\Delta\to X$ holomorphic, with $\phi(\zeta)=z$ and
$\phi(\eta)=w$}\}
$$
for all $z$, $w\in X$. The {\sl Kobayashi pseudodistance}~$k_X\colon X\times X\to\R^+$ of~$X$
is the largest pseudodistance on~$X$ bounded above by~$\delta_X$. We say that $X$ is
{\sl (Kobayashi) hyperbolic} if $k_X$ is a true distance --- and in that case it is known that the
metric topology induced by~$k_X$ coincides with the manifold topology of~$X$ (see, e.g., [A2, Proposition~2.3.10]). For instance, all bounded domains are hyperbolic (see, e.g., [A2, Theorem~2.3.14]).

The main property of the Kobayashi (pseudo)distance is that it is contracted by holomorphic maps: if $f\colon X\to Y$ is a holomorphic map then
$$
\forevery{z,w\in X} k_Y\bigl(f(z),f(w)\bigr)\le k_X(z,w)\;.
$$
In particular, the Kobayashi distance is invariant under biholomorphisms.
%, and decreases under inclusions:
%if $D_1\subset D_2\subset\subset\C ^n$ are two bounded domains we have 
%$k_{D_2}(z,w)\le k_{D_1}(z,w)$ for all $z$,~$w\in D_1$.

It is easy to see that the Kobayashi distance of the unit disk coincides with the Poincar\'e distance.
Furthermore, the Kobayashi distance of the unit ball $B^d\subset\C^d$ coincides with the
Bergman distance (see, e.g., [A2, Corollary~2.3.6]); and the Kobayashi distance of a bounded
convex domain coincides with the Lempert function (see, e.g., [A2, Proposition~2.3.44]). Moreover, the Kobayashi distance of a bounded convex domain $D$ is complete ([A2, Proposition~2.3.45]), and thus
for each $p\in D$ we have that $k_D(p,z)\to+\infty$ if and only if $z\to\de D$.

A {\sl complex geodesic} in a hyperbolic manifold~$X$ is a holomorphic map
$\phe\colon\Delta\to X$ which is an isometry with respect to the Kobayashi distance of~$\Delta$
and the Kobayashi distance of~$X$. Lempert's theory (see [L] and [A2, Chapter~2.6]) of
complex geodesics in strongly convex domains is one of the main tools for the study of
the geometric function theory of strongly convex domains. In particular, we shall need the
following facts, summirizing Lempert's and Royden-Wong's theory, valid for any bounded convex domain $D\subset\subset\C^d$:
\smallskip
\item{(a)} [A2, Theorem~2.6.19 and Corollary~2.6.30] for every pair of distinct points $z$, $w\in D$ there exists a complex geodesic
$\phe\colon\Delta\to D$ such that $\phe(0)=z$ and $\phe(r)=w$, where $0<r<1$ is such that
$k_\Delta(0,r)=k_D(z,w)$; furthermore, if $D$ is strongly convex then $\phe$ is unique;
\item{(b)} [A2, Theorem~2.6.19] a holomorphic map $\phe\in\Hol(\Delta,D)$ is a complex
geodesic if and only if $k_D\bigl(\phe(\zeta_1),\phe(\zeta_2)\bigr)=k_\Delta(\zeta_1,\zeta_2)$
for a pair of distinct points $\zeta_1$, $\zeta_2\in\Delta$;
\item{(c)} [A2, Proposition~2.6.22] every complex geodesic $\phe\in\Hol(\Delta,D)$ admits
a {\sl left inverse,} that is a holomorphic map $\tilde p_\phe\colon D\to\Delta$ such that
$\tilde p_\phe\circ\phe=\id_\Delta$; the map $p_\phe=\phe\circ\tilde p_\phe$ is then 
a holomorphic retraction of $D$ onto the image of~$\phe$;
\item{(d)} [A2, Theorem~2.6.29] if $D$ is strongly convex of class~$C^2$, then every
complex geodesics extend continuously (actually, ${1\over 2}$-H\"older) to the boundary of~$\Delta$, and the image of $\phe$ is transversal to~$\de D$;
\item{(e)} [A2, Theorem~2.6.45] if $D$ is strongly convex and of class~$C^2$, then for every
$z\in D$ and $\tau\in\de D$ there is a complex geodesic $\phe\in\Hol(\Delta,D)$ with
$\phe(0)=z$ and $\phe(1)=\tau$; and for every pair of distinct points $\sigma$, $\tau\in\de D$
there is a complex geodesic $\phe\in\Hol(\Delta,D)$ such that $\phe(-1)=\sigma$ and
$\phe(1)=\tau$. (The statement of [A2, Theorem~2.6.45] requires $D$ of class $C^3$, but the
proof of the existence works assuming just $C^2$ smoothness.)
\smallskip

Now let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$ a holomorphic self-map of $D$. As mentioned in the introduction, if the set $\Fix(f)$ of fixed
points of $f$ in~$D$ is not empty, then (see [A1, 2, 3]) the sequence $\{f^n\}$ of iterates of~$f$ is relatively
compact in~$\Hol(D,D)$, and 
there exists a submanifold $D_0\subseteq D$, the {\sl limit manifold}
of~$f$, such that every limit of a subsequence of iterates is of the form $\gamma\circ\rho$,
where $\rho\colon D\to D_0$ is a holomorphic retraction, and $\gamma$ is a biholomorphism
of~$D_0$; furthermore, $f|_{D_0}$ is a biholomorphism of~$D_0$, and $\Fix(f)\subseteq D_0$. 

\newdef
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain. A holomorphic map 
$f\in\Hol(D,D)$ is {\sl elliptic} if $\Fix(f)\ne\void$; and {\sl strongly elliptic} if its limit manifold
reduces to a point (called the {\sl Wolff point} of the strongly elliptic map). We shall say that a point $p\in\Fix(f)$ is {\sl attracting} if all the 
eigenvalues of $df_p$ have modulus less than 1.

Later on we shall need an equivalent characterization of strongly elliptic maps:

\newthm
Lemma \uunoa:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$.
Then the following facts are equivalent:
\smallskip
\itm{(i)} $f$ is strongly elliptic;
\itm{(ii)} the sequence of iterates of $f$ converges to a point $p\in D$;
\itm{(iii)} $f$ has an attracting fixed point $p\in D$;
\itm{(iv)} there exists $p\in\Fix(f)$ such that $k_D\bigl(p,f(z)\bigr)< k_D(p,z)$ for all $z\in D\setminus\{p\}$.

\pf The equivalence of (i), (ii) and (iii) is well-known, and more generally valid in taut manifolds
(see, e.g., [A2, Corollary~2.4.2]). 

Now, if $f$ is not strongly elliptic, the limit manifold $D_0$ has positive dimension. Being a
holomorphic retract of~$D$, the Kobayashi distance of~$D_0$ coincides with the restriction of
Kobayashi distance of~$D$; hence $k_D\bigl(f(z),f(w)\bigr)=k_D(z,w)$ for all $z$,~$w\in D_0$,
because $f|_{D_0}$ is a biholomorphism of~$D_0$ (and thus an isometry for the Kobayashi
distance). Since $\Fix(f)\subseteq D_0$, this shows that (iv) implies (i).

Finally, assume that (iv) does not hold, and thus there are $p\in\Fix(f)$ and $z_0\in D\setminus\{p\}$ with $k_D\bigl(p,f(z_0)\bigr)= k_D(p,z_0)$. Let $\phe\in\Hol(\Delta,D)$ be a complex geodesic
with $\phe(0)=p$ and $\phe(r)=z_0$, for a suitable $0<r<1$. Then 
$$
k_D\bigl(p,f\bigl(\phe(r)\bigr)\bigr)=k_D(p,z_0)=k_\Delta(0,r)\;;
$$
since $f(p)=p$ this implies that $f\circ\phe$ is still a complex geodesic. Since complex 
geodesics are also infinitesimal isometries with respect to the Kobayashi metric (see [A2, Corollary~2.6.20]), the Kobayashi length of $\phe'(0)$ must be equal to the Kobayashi length
of $(f\circ\phe)'(0)=df_p\bigl(\phe'(0)\bigr)$. In particular, $p$ cannot be an attracting
fixed point, and thus $f$ cannot be strongly elliptic.
\qedn

In the study of the dynamics of self-maps without fixed points, a crucial role is played by the
horospheres, a generalization (introduced in [A1]) of
the classical notion of horocycle. Let $D\subset\subset\C^d$ be a 
bounded strongly convex $C^2$ domain. For every $\tau\in\de D$ and $p\in D$
let $h_{\tau,p}\colon D\to\R^+$ be given by
$$
\mlog h_{\tau,p}(z)=\lim_{w\to\tau}[k_D(z,w)-k_D(p,w)]\;;
$$
notice that the existence of the limit is a 
non-trivial fact (see [A1, Theorem~2.6.47] or [BP]). Then
the {\sl horosphere} of {\sl center} $\tau\in\de D$,
{\sl radius} $R>0$ and {\sl pole} $p\in D$ is the set
$$
E_p(\tau,R)=\{z\in D\mid h_{\tau,p}(z)< R\}\;.
$$
It is well-known (see, again, [A1], [A2] and [BP]) that the horospheres
with pole at the origin in the unit disk $\Delta\subset\C$ coincide with the classical horocycles,
that the horospheres with pole at the origin in the unit ball $B^n\subset\C^n$ again coincide
with the usual horospheres, and that the horospheres in strongly convex domains are convex. Furthermore, the closure of a horosphere intersects the boundary of~$D$
exactly in the center of the horosphere; and the shape of a horosphere near the boundary is
comparable to the shape of the horospheres in the ball, that is, they are close to be ellipsoids.
An easy observation we shall need later on is that changing the pole amounts to multiplying the radius by a fixed 
constant:

\newthm
Lemma \chtp:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $\tau\in\de D$.
Then
$$
h_{\tau,q}={1\over h_{\tau,p}(q)}h_{\tau,p}
$$
for all $p$, $q\in\ D$. In particular,
$$
\forevery{R>0} E_q(\tau,R)=E_p\bigl(\tau, h_{\tau,p}(q)R\bigr)\;.
$$

\pf
It suffices to write
$$
k_D(z,w)-k_D(q,w)=[k_D(z,w)-k_D(p,w)]-[k_D(q,w)-k_D(p,w)]\;,
$$
and let $w\to\tau$.
\qedn

In a similar way we can introduce $K$-regions. Let $D\subset\subset\C^d$ be a 
bounded strongly convex $C^2$ domain.  The {\sl $K$-region} $K_p(\tau,M)$ of 
of {\sl center} $\tau\in\de D$,
{\sl amplitude} $M>0$ and {\sl pole} $p\in D$ is the set
$$
K_p(\tau,M)=\{z\in D\mid \mlog h_{\tau,p}(z)+k_D(p,z)< \log M\}\;.
$$
It is well-known (see [A2] or [A3]) that the $K$-regions
with pole at the origin in the unit disk coincide with the classical Stolz regions,
and that the $K$-regions with pole at the origin in the unit ball $B^n\subset\C^n$ coincide
with the usual Kor\'anyi approach regions. Furthermore, in strongly convex domains
$K$-regions are comparable to Stein admissible regions; and changing the pole does not
change much the $K$-regions, because ([A2, Lemma~2.7.2]) for each $p$,~$q\in D$ there is $L>0$ such that
$$
K_p(\tau, M/L)\subseteq K_q(\tau,M)\subseteq K_p(\tau,ML)
\neweq\eqKpole
$$
for every $M>0$.
Given $\tau\in\de D$, we shall say that a function $F\colon D\to\C^n$ has {\sl $K$-limit}
$\ell\in\C^n$ at~$\tau$ if $F(z)\to\ell$ as $z\to\tau$ inside any $K$-region centered at~$\tau$;
notice that the choice of the pole is immaterial because of \eqKpole. Since $K$-regions
in strongly convex domains
are comparable to Stein admissible regions, the notion of $K$-limit is equivalent to 
Stein admissible limit, and thus it is the right generalization to several variables of the
one-dimensional notion of non-tangential limit (in particular, the existence of a $K$-limit always
implies the existence of a non-tangential limit). Finally, the intersection of a horosphere (or $K$-region) of center~$\tau\in\de D$ and pole~$p\in D$ with the image of a complex geodesic~$\phe$
with $\phe(0)=p$ and $\phe(1)=\tau$ is the image via~$\phe$ of the horosphere (or $K$-region)
of center~1 and pole~0 in the unit disk ([A2, Proposition~2.7.8 and Lemma~2.7.16]).

The correct generalization of  the one-variable notion of angular derivative is given by the
dilation coefficient (see [A2, Section~1.2.1 and Theorem~2.7.14]):

\newdef
Take $f\in\Hol(D,D)$, where again $D\subset\subset\C^d$ is 
a bounded strongly convex $C^2$ domain, and let $\sigma\in\de D$. The {\sl dilation coefficient} $\beta_{\sigma,p}\in(0,+\infty]$
of $f$ at~$\sigma\in\de D$ with pole~$p\in D$ is given by
$$
\mlog\beta_{\sigma,p}=\liminf_{z\to\sigma}\bigl[k_D(p,z)-k_D\bigl(p,f(z)\bigr)\bigr]\;.
$$
Furthermore, $\sigma\in\de D$ is a {\sl boundary fixed point}
of~$f$ if $f$ has $K$-limit $\sigma$ at~$\sigma$. 

Since
$$
k_D(p,z)-k_D\bigl(p,f(z)\bigr)\ge k_D\bigl(f(p),f(z)\bigr)-k_D\bigl(p,f(z)\bigr)\ge -k_D\bigl(p,f(p)\bigr)\;,
$$
the dilation coefficient cannot be zero. We also recall
the following useful formulas for computing the dilation coefficient ([A2, Lemma~2.7.22]):
$$
\mlog\beta_{\sigma,p}=\lim_{t\to 1}\bigl[k_D\bigl(p,\phe(t)\bigr)-k_D\bigl(p,f\bigl(\phe(t)\bigr)\bigr)
\bigr]=\lim_{t\to 1}\bigl[k_D\bigl(p,\phe(t)\bigr)-k_D\bigl(p,p_\phe\circ f\bigl(\phe(t)\bigr)\bigr)
\bigr]\;,
\neweq\equsf
$$
where $\phe\in\Hol(\Delta,D)$ is a complex geodesic with $\phe(0)=p$ and $\phe(1)=\sigma$,
and $p_\phe=\phe\circ\tilde p_\phe$ is the holomorphic retraction associated to~$\phe$.

When $\sigma$ is a boundary fixed point then the dilation coefficient does not depend
on the pole:

\newthm
Lemma \dcp:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, $f\in\Hol(D,D)$
and $\sigma\in\de D$ a boundary fixed point of~$f$. Then $\beta_{\sigma,p}=\beta_{\sigma,q}$ for all $p$,~$q\in D$.

\pf 
If the dilation coefficient is infinite for all poles we are done.
Assume there is $p\in D$ such that the dilation coefficient $\beta_{\sigma,p}$ is finite.
Given $q\in D$, write 
$$
\eqalign{k_D(q,z)&-k_D\bigl(q,f(z)\bigr)\cr
&=k_D(p,z)-k_D\bigl(p,f(z)\bigr)+\bigl[k_D(q,z)-k_D(p,z)\bigr]
+\bigl[k_D\bigl(p,f(z)\bigr)-k_D\bigl(q,f(z)\bigr)\bigr]\;.\cr}
\neweq\eqdcpu
$$
The first term inside square brackets converges to $\mlog h_{\sigma,p}(q)$ when $z\to\sigma$.
Now, let $\phe\in\Hol(\Delta,D)$ be a complex geodesic with $\phe(0)=p$ and 
$\phe(1)=\sigma$. Since $\phe(t)\to\sigma$ non-tangentially as $t\to 1^-$, we have
$f\bigl(\sigma(t)\bigr)\to\sigma$. Therefore if we put $z=\phe(t)$ in \eqdcpu, letting $t\to 1^-$ and recalling \equsf\ we get
$$ 
\mlog \beta_{\sigma,q}\le \mlog \beta_{\sigma,p}+\mlog h_{\sigma,p}(q)-\mlog h_{\sigma,p}(q)=
\mlog\beta_{\sigma,p}\;.
$$
Thus $\beta_{\sigma,q}$ is finite too, and reversing the roles of $p$ and $q$ we get the assertion.
\qedn

In particular, we shall simply denote by $\beta_\sigma$ the dilation coefficient at a boundary fixed point.

\newdef
Let $\sigma\in\de D$ be a boundary fixed point for a self-map $f\in\Hol(D,D)$ of
a bounded strongly convex $C^2$ domain $D\subset\subset\C^d$. We shall say that 
$\sigma$ is {\sl attracting} if $0<\beta_\sigma<1$, {\sl parabolic} if $\beta_\sigma=1$
and {\sl repelling} if $\beta_\sigma>1$.

We can now quote the general versions of Julia's lemma proved in [A1, 3] (see [A2, Theorem~2.4.16 and Proposition~2.7.15]) that we shall need
in this paper:

\newthm 
Proposition \Julia: (Abate, 1988)
Let $D\subset\subset\C^n$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$. Let $\sigma\in\de D$ and $p\in D$ be such that the dilation coefficient $\beta_{\sigma, p}$ is finite.
Then there exists a unique $\tau\in\de D$ such that
$$
\forevery{R>0} f\bigl(E_p(\sigma,R)\bigr)\subseteq E_p\bigl(\tau,\beta_{\sigma,p}R\bigr)\;,
$$
and $f$ has $K$-limit $\tau$ at~$\sigma$. 

Finally, we recall the several variable version of the Wolff-Denjoy theorem given in~[A1]
(see [A2, Theorems~2.4.19 and~2.4.23]):

\newthm
Theorem \Wolff: (Abate, 1988)
Let $D\subset\subset\C^n$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$
without fixed points. Then there exists a unique $\tau\in\de D$ such that the sequence of
iterates of $f$ converges to~$\tau$. 

\newdef
Let $D\subset\subset\C^n$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$
without fixed points. The point $\tau\in\de D$ introduced in the previous theorem is the
{\sl Wolff point} of~$f$. 

The Wolff point can be characterized by the dilation coefficient:

\newthm 
Proposition \AcW: 
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$ without fixed points in~$D$. Then the
following assertions are equivalent for a point $\tau\in\de D$:
\smallskip
\itm{(i)} $\tau$ is a boundary fixed point with $0<\beta_\tau\le 1$;
\itm{(ii)} $f\bigl(E_p(\tau,R)\bigr)\subseteq E_p(\tau,R)$ for all $R>0$ and any (and hence all) $p\in D$;
\itm{(iii)} $\tau$ is the Wolff point of $f$.

\pf 
(i)${}\Longrightarrow{}$(ii): it follows immediately from Proposition~\Julia.

(ii)${}\Longrightarrow{}$(iii): it follows, as in the proof of [A2, Theorem~2.4.23], from the facts that
the sequence of iterates $\{f^n\}$ is compactly divergent and that $\bar{E_p(\tau,R)}\cap\de D=\{\tau\}$ for all $R>0$ and $p\in D$.

(iii)${}\Longrightarrow{}$(i): since $f$ has no fixed points, by [A2, Theorem~2.4.19] there is
a $\tau'\in\de D$ such that $f\bigl(E_p(\tau',R)\bigr)\subseteq E_p(\tau',R)$ for all $R>0$
and $p\in D$. Since $\bar{E_p(\tau',R)}\cap\de D=\{\tau'\}$ we must have $\tau'=\tau$.
Now fix $p\in D$ and let $\phe\in\Hol(\Delta,D)$ be a complex geodesic with 
$\phe(0)=p$ and $\phe(1)=\tau$. Let $\tilde p_\phe\in\Hol(D,\Delta)$ be the left inverse
of~$\phe$, and put $\tilde f=\tilde p_\phe\circ f\circ\phe\in\Hol(\Delta,\Delta)$. 
Since, as observed before, complex geodesics and left-inverses preserve the horospheres
(see [A2, Proposition~2.7.8 and Lemma~2.7.16]), we have $\tilde f\bigl(E_0(1,R)\bigr)\subseteq
E_0(1,R)$ for all $R>0$. This easily implies that either $\tilde f$ has no fixed points
or it is the identity. In the latter case \equsf\ implies that $\beta_\tau=1$, and
we are done. 

If instead $\tilde f$ has no fixed points, by the one-variable Wolff's lemma, $1\in\de\Delta$ is its Wolff point, and ([A2, Corollary~1.2.16]) the dilation coefficient $\beta$ of $\tilde f$ at~1 belongs to~$(0,1]$.
But, again by \equsf, $\beta=\beta_\tau$, and we are done.
\qedn

\newdef
Let $D\subset\subset\C^n$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$
without fixed points and with Wolff point $\tau\in\de D$. 
We shall say that $f$ is {\sl hyperbolic} if $0<\beta_\tau<1$
and {\sl parabolic} if $\beta_\tau=1$.


\smallsect 2. Convergence of backward orbits

In this section we shall prove our main Theorem~\OJMz. This will be accomplished by a
sequence of lemmas, but first we recall 
a couple of definitions:

\newdef 
Let $f\colon X\to X$ be a self-map of a set $X$. A {\sl backward orbit} (or {\sl backward iteration sequence\/}) for~$f$ is a sequence
$\{x_n\}_{n\in\N}\subset X$ so that $f(x_{n+1})=x_n$ for all $n\in\N$.

\newdef
Let $X$ be a (Kobayashi) hyperbolic manifold. We say that a sequence $\{z_n\}\subset X$ has
{\sl bounded Kobayashi step} if 
$$
a=\sup\limits_n k_X(z_{n+1},z_n)<+\infty\;.
$$ 
The number~$a$ is
the {\sl Kobayashi step} of the sequence.

%
%\newthm 
%Theorem \OJM:
%Let $D\subset\subset\C^d$ be a bounded smooth strongly convex domain.
%Let $f\in\Hol(D,D)$ be either hyperbolic, parabolic, or strongly elliptic, with Wolff point $\tau\in\bar{D}$. 
%Let $\{z_n\}\subset D$ be a backward iteration sequence for~$f$ with bounded Kobayashi step~$a>0$.
%Then:
%\item{\rm (i)}there exists a point~$\sigma\in\de D$ such that $z_n\to\sigma$ as~$n\to+\infty$;
%\item{\rm (ii)} there exists $M>0$ so that $z_n\in K_{p}(\sigma,M)$ eventually, where $p$ is any point in $D$, if $f$ is hyperbolic or parabolic, or $p$ is the unique fixed point of $f$, if $f$ is strongly elliptic; 
%\item{\rm (iii)} if $\sigma = \tau$, then $f$ is parabolic;
%\item{\rm (iv)} there exists $\alpha\ge 1$ such that
%$$
%f\bigl(E_{p}(\sigma,R)\bigr)\subseteq E_{p}(\sigma,\alpha R)
%$$ 
%for all $R>0$, where $p$ is any point in $D$, if $f$ is hyperbolic or parabolic, or $p$ is the unique fixed point of $f$, if $f$ is strongly elliptic.\sm

We shall first deal with the hyperbolic and parabolic cases.

\newthm
Lemma \uundici:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain. Let $\{z_n\}\subset D$ be a backward orbit for a  parabolic or hyperbolic self-map $f\in\Hol(D,D)$. 
Then $z_n\to\de D$ as $n\to+\infty$. 

\pf
Assume, by contradiction, that the sequence does not converge to $\de D$. Then there exists a subsequence $\{z_{n_k}\}$ converging to $w_0\in D$, that is, such that 
$$
k_D(w_0,z_{n_k}) \to 0 \quad \hbox{as}~k\to +\infty\;.
$$
Therefore
$$
k_D\bigl(f^{n_k}(w_0), f^{n_k}(z_{n_k})\bigr) \le k_D(w_0,z_{n_k}) \to 0 \quad \hbox{as}~k\to +\infty\;.
$$
But, on the other hand, $f^{n_k}(z_{n_k}) = z_0$ for all $k$; moreover,
$f^{n_k}(w_0) \to\tau$ as $k\to+\infty$, where $\tau\in\de D$ is the Wolff point of~$f$, and so
$$
\lim_{k\to\infty}k_D\bigl(f^{n_k}(w_0), f^{n_k}(z_{n_k})\bigr) = +\infty\;,
$$
because $k_D$ is complete, contradiction.
\qedn

\newthm
Lemma \udue:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain. Let $\{z_n\}\subset D$ be
a sequence with bounded Kobayashi step $a>0$ converging toward the boundary of~$D$.
Then there exists $\sigma\in\de D$ such that $z_n\to\sigma$ as~$n\to+\infty$.

\pf
Since $z_n\to\de D$, we can find a subsequence $\{z_{n_j}\}$ converging to a point~$\sigma\in\de D$; we claim that the whole sequence converges to~$\sigma$.

If for every $k\in\N$ the subsequence $\{z_{n_j+k}\}$ converges to~$\sigma$, then clearly the
whole sequence converges to~$\sigma$ and we are done. Otherwise, there exists a minimum $k>0$ such that
the sequence $\{z_{n_j+k-1}\}$ converges to~$\sigma$ but $\{z_{n_j+k}\}$ does not. 
Up to extracting a subsequence in both and renaming, we may then assume that 
$\{z_{n_j}\}$ converges to~$\sigma$ while $\{z_{n_j+1}\}$ converges to $\widetilde\sigma\in\de D$ different
from~$\sigma$.

Then [A2, Corollary~2.3.55] yields $\eps>0$ and $K>0$ such that, as soon as $\|z_{n_j}-\sigma\|<\eps$,
and $\|z_{n_j+1}-\widetilde\sigma\|<\eps$, we have
$$
K-\mlog d(z_{n_j},\de D)-\mlog d(z_{n_j+1},\de D)\le k_D(z_{n_j},z_{n_j+1})\le a\;.
$$
Letting $j\to+\infty$ we get a contradiction.
\qedn

%Inductively, we obtain that $z_n\notin E_p(\tau,c_p^{-n}t_0)$ for all $n>0$. Since
%$$
%E_p(\tau,t_0)\subset E_p(\tau, c_p^{-1}t_0)\subset\cdots\subset E_p(\tau, c_p^{-n}t_0)\subset\cdots
%$$
%and 
%$$
%\bigcup_{n\in\N} E_p(\tau, c_p^{-n}t_0)=D
%$$
%because $c_p<1$, it follows that $\{z_n\}$ cannot have limit points in~$D$.
%\qedn


\newthm 
Lemma \utre:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and fix $p\in D$.
Let $f\in\Hol(D,D)$, and 
$\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step~$a=\mlog\alpha$ converging to~$\sigma\in\de D$. Then $\sigma$ is a boundary fixed point of~$f$ and 
$\beta_\sigma\le\alpha$. 
%$$
%\forevery{R>0} f\bigl(E_p(\sigma,R)\bigr)\subseteq E_p(\sigma,\alpha R)\;.
%$$

\pf 
Fix $p\in D$. 
First of all we have 
$$
\eqalign{
\mlog\beta_{\sigma,p}=\liminf_{w\to\sigma}\bigl[k_D(w,p)-k_D\bigl(f(w),p\bigr)\bigr]&\le \liminf_{n\to+\infty}
[k_D(z_{n+1},p)-k_D\bigl(z_n,p\bigr)]\cr
&\le \liminf_{n\to+\infty} k_D(z_{n+1},z_n)\cr
&\le a=\mlog\alpha\;.
\cr}
$$
Since $z_n\to\sigma$ and $f(z_n)=z_{n-1}\to\sigma$ as $n\to+\infty$, using [A2, Proposition~2.4.15] we get
that $f\bigl(E_p(\sigma,R)\bigr)\subseteq E_p(\sigma,\alpha R)$ for all~$R>0$.
Then Proposition~\Julia\  implies that $f$ has $K$-limit $\sigma$ at~$\sigma$,
and we are done.
\qedn

\newthm
Lemma \uqua:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be hyperbolic or parabolic with Wolff point $\tau\in\de D$
and dilation coefficient~$0<\beta_\tau\le 1$. 
Let $\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step converging to~$\sigma\in\de D\setminus\{\tau\}$. Then
$$
\beta_\sigma\ge {1\over \beta_\tau}\ge 1\;.
$$

\pf 
Let $\phe\colon\bar{\Delta}\to\bar{D}$ be a complex geodesic such that
$\phe(-1)=\sigma$ and $\phe(1)=\tau$, and set $p=\phe(0)$. 
Proposition~\Julia\ yields
$$
p\in \bar{E_p(\sigma,1)}\qquad\Longrightarrow\qquad f(p)\in\bar{E_p(\sigma,\beta_\sigma)}
$$
and 
$$
p\in \bar{E_p(\tau,1)}\qquad\Longrightarrow\qquad f(p)\in\bar{E_p(\tau,\beta_\tau)}\;.
$$
Hence $\bar{E_p(\sigma,\beta_\sigma)}\cap\bar{E_p(\tau,\beta_\tau)}\ne\void$. 

Let $\tilde p_\phe\colon D\to\Delta$ be the left-inverse of~$\phe$. Then
$$
\eqalign{
\void&\ne \tilde p_\phe\left(\bar{E_p(\sigma,\beta_\sigma)}\cap\bar{E_p(\tau,\beta_\tau)}\right)
	\subseteq\tilde p_\phe(\bar{E_p(\sigma,\beta_\sigma)})\cap \tilde p_\phe(\bar{E_p(\tau,\beta_\tau)})\cr
	&= \bar{E_0(-1,\beta_\sigma)}\cap \bar{E_0(1,\beta_\tau)}\;.\cr}
$$  
Now, $E_0(1,\beta_\tau)$ is an Euclidean disk of radius~$\beta_\tau/(\beta_\tau+1)$ tangent to~$\de\Delta$
in~$1$, and $E_0(-1,\beta_\sigma)$ is an Euclidean disk of radius~$\beta_\sigma/(\beta_\sigma+1)$ tangent to~$\de\Delta$
in~$-1$. So these disks intersect if and only if
$$
1-{2\beta_\tau\over \beta_\tau+1}\le -1+{2\beta_\sigma\over\beta_\sigma+1}\;,
$$
which is equivalent to $\beta_\sigma \beta_\tau\ge 1$, as claimed.
\qedn

In this way we proved Theorem~\OJMz.(i) for hyperbolic and parabolic maps.
Now we prove Theorem~\OJMz.(iv):

\newthm
Lemma \udieci:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and fix $p\in D$.
Let $f\in\Hol(D,D)$ be hyperbolic or parabolic with Wolff point $\tau\in\de D$, and let
$\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step $a=\mlog\alpha$ converging to~$\sigma\in\de D$. Then for every $p\in D$ 
there exists $M>0$ such that $z_n\in K_{p}(\sigma,M)$ eventually. 

\pf
Choose $p\in M$.
%Let $\phe\colon\bar{\Delta}\to\bar{D}$ be a complex geodesic such that
%$\phe(-1)=\sigma$ and $\phe(1)=\tau$; by \eqKpole\ it suffices to prove the
%assertion for $p=\phe(0)$.
% and let $p_\phe\colon\bar{D}\to\bar\Delta$ be the left-inverse of~$\phe$. 
We clearly have
 $$
 \liminf_{n\to \infty} [k_D(p,z_{n+1}) - k_D(p,z_n)]\ge \mlog\beta_\sigma\;;%\ge\mlog{1\over\beta_\tau}\;;
 $$
%Set
%$$
%\mlog\beta := \liminf_{z\to \sigma} [k_D(p,z) - k_D(p,f(z))]\le\liminf_{n\to \infty} [k_D(p,z_{n+1}) - k_D(p,z_n)] \;.
%$$
%Thanks to Julia-Wolff-Caratheodory, we have
%$$
%\beta = \lim_{\zeta\to -1} {d\over d\zeta}\left( P_\phe(f(\phe(\zeta)))\right)
%$$
%and by Julia's Lemma we have 
%$$
%P_\phe(f(\phe(E_\Delta(-1, R)))) \subset E_\Delta(-1,\beta R)\quad\hbox{and}\quad P_\phe(f(\phe(E_\Delta(1, R)))) \subset E_\Delta(1,c_p R)\;,
%$$
%and hence, by Lemma~\uqua, we obtain
%$$
%\beta \ge {1\over c_p} \ge 1\;.
%$$
since, by the previous lemma, $\beta_\sigma\ge 1$, 
there thus exists $n_0\ge 0$ such that
$$
k_D(p,z_{n+1}) - k_D(p,z_n)\ge \mlog \beta_\sigma^{1/2}
$$
for all $n\ge n_0$.
%perche' $\liminf_{n\to \infty} [k_D(p,z_{n+1}) - k_D(p,z_n)]\ge {1\over 2} \log {1\over c_p}$
Therefore
$$
k_D(p,z_{n+1}) - k_D(p,z_n) - k_D(z_{n+1},z_n)\ge \mlog \beta_\sigma^{1/2} - \mlog \alpha> - \infty\;, 
$$
and hence
$$
\eqalign{
k_D(p,z_{n+2}) - k_D(p,z_n) - k_D(z_{n+2},z_n)
&\!\ge\! k_D(p,z_{n+1}) - k_D(z_{n+2},z_{n+1}) - k_D (p, z_n) - k_D(z_{n+2},z_n)\cr
&\!\ge\! k_D(p,z_{n+1}) - k_D (p, z_n) - k_D(z_{n+1},z_n)\cr
&\!\ge\! \mlog {\beta_\sigma^{1/2}\over \alpha}\;.
}
$$
By induction, for any $m>n\ge n_0$ we thus have
$$
k_D(p,z_m) - k_D(p,z_n) - k_D(z_m,z_n)\ge \mlog {\beta_\sigma^{1/2}\over \alpha}\;,
$$
i.e.,
$$
k_D(z_m,z_n) - k_D(p,z_m)+k_D(p,z_n) \le \mlog \left(\alpha\beta_\sigma^{-1/2}\right)\;.
$$
Then 
$$
\eqalign{
\lim_{w\to\sigma}[k_D(z_n,w) - k_D(p, w)] + k_D(p, z_n) 
&= \lim_{m\to\infty}[k_D(z_n,z_m) - k_D(p, z_m)] + k_D(p, z_n) \cr
&\le \mlog \left(\alpha \beta_\sigma^{-1/2}\right)<+\infty\;,
}
$$
for all $n\ge n_0$, and we are done.
\qedn

To prove Theorem~\OJMz.(iii) we need another lemma:

\newthm
Lemma \uuno:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and fix $p\in D$.
Let $f\in\Hol(D,D)$ be hyperbolic or parabolic with Wolff point $\tau\in\de D$ and dilation coefficient
$0<\beta_\tau\le 1$. 
Let $\{z_n\}\subset D$ be a backward orbit for~$f$. Then 
$$
\forevery{n\in\N}
h_{\tau,p}(z_n)\ge \left({1\over\beta_\tau}\right)^n h_{\tau,p}(z_0)\;.
$$

\pf
Put $t_n=h_{\tau,p}(z_n)$.
By definition, 
$z_n\in\de E_{p}(\tau,t_n)$. By Proposition~\Julia, if $z_{n+1}\in
E_{p}(\tau,R)$ then $z_n\in E_{p}(\tau,\beta_\tau R)$. Since $z_n\notin  E_{p}(\tau,t_n)$, we
have that $z_{n+1}\notin E_{p}(\tau, \beta_\tau^{-1}t_n)$, that is
$$
t_{n+1}\ge {1\over \beta_\tau}\, t_n\;,
\neweq\equuno
$$
and the assertion follows by induction.
\qedn

\newthm
Corollary \udodici:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain. Let $f\in\Hol(D,D)$ be hyperbolic with Wolff point $\tau\in\bar{D}$. 
Let $\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step~$a>0$
converging to $\sigma\in \de D$. Then $\sigma \ne \tau$.

\pf
By Lemma~\udieci, the sequence $\{z_n\}$ converges to $\sigma$ inside a Kor\'anyi region
with center~$\sigma$. But, by Lemma~\uuno, $z_n$ is eventually outside any horosphere centered in $\tau$, and this clearly implies $\tau\ne \sigma$ as claimed.
\qedn

So we have Theorem~\OJMz.(iii), and together with Lemma~\uqua\ we also proved
Theorem~\OJMz.(ii) for the hyperbolic case.

\newrem
Lemma~\uuno\ can be used to give another proof of the convergence of a backward orbit of bounded
Kobayashi step for hyperbolic maps. First of all, [AS, Remark~3] 
yields a constant $C_1>0$ such that
$$
\|z_n-z_{n+1}\|\le {C_1\over\sqrt{1-\hat a^2}}\sqrt{d(z_n,\de D)}\le {C_1\over 1-\hat a}\sqrt{d(z_n,\de D)}\;,
\neweq\eqAS
$$
where $\hat a=\tanh a\in(0,1)$ and $a$ is the Kobayashi step of the backward orbit $\{z_n\}$.
On the other hand, given $p\in D$
the triangular inequality and the upper estimate [A2, Theorem~2.3.51] on the boundary behavior of the Kobayashi distance yield a constant $C_2>0$ such that
$$
\mlog h_{\tau,p}(z_n)\le k_D(p,z_n)\le C_2-\mlog d(z_n,\de D)\;,
$$ 
%that is
%$$
%d(z_n,\de D)\le {e^{2C_2}\over h_{\tau,p}(z_n)}\;,
%\neweq\eqestup
%$$
and thus
$$
\|z_n-z_{n+1}\|\le {C\over 1-\hat a}\sqrt{{1\over h_{\tau,p}(z_n)}}\;,
\neweq\equotto
$$
for a suitable $C>0$. Therefore using Lemma~\uuno\ we get that for every
$m\ge n\ge 0$ we have
$$
\|z_m-z_n\|\le\sum_{j=n}^{m-1}\|z_{j+1}-z_j\|\le{C\over 1-\hat a}{1\over\sqrt{h_{\tau,p}(z_0)}}
\sum_{j=n}^{m-1} \beta_\tau^{j/2}\le{C\over 1-\hat a}{1\over 1-\beta_\tau^{1/2}}{\beta_\tau^{n/2}\over\sqrt{h_{\tau,p}(z_0)}}\;,
$$
and so $\{z_n\}$ is a Cauchy sequence in~$\C^d$, converging to a point $\sigma\in\de D$ by Lemma~\uundici.

%where $\hat a\in(0,1)$ is given by $\hat a=\tanh a$ and
%$t_n>0$ is defined by
%$$
%\mlog t_n=\lim_{w\to\tau}[k_D(w,z_n)-k_D(w,p)]\;.
%$$
%
%\pf
%By assumption, we have $k_D(z_n,z_{n+1})\le a$ for all $n\in\N$. Therefore
%Lemma~2.4 and Remark~3 of [Abate-Saracco] %%and we are done.


% Indeed, in the hyperbolic case \equuno\ and \equotto\ imply that  In the strongly elliptic case the same
%argument works using \equsei\ instead of \equuno\ and \equnove\ instead of \equotto.


Let us now deal with strongly elliptic maps. We need a preliminary lemma:

\newthm
Lemma \ucin:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be strongly elliptic with Wolff point $p\in D$. Then for every $R_0>0$
there exists $0<c=c(R_0)<1$ such that 
$$
k_D\bigl(f(z),p\bigr)-k_D(z,p)\le \mlog c<0
$$
for all $z\in D$ with $k_D(z,p)\ge R_0$. 

\pf
By contradiction, assume that for every $c<1$ there exists $z(c)\in D$ with $k_D\bigl(z(c),p\bigr)\ge R_0$ so that 
$$
k_D\bigl(f\bigl(z(c)\bigr),p\bigr)-k_D\bigl(z(c),p\bigr)> \mlog c\;.
$$
Let $z_\infty\in\bar D$ be a limit point of the sequence $\{z(1-1/n)\}$. If $z_\infty\in D$ then
$$
k_D\bigl(f\bigl(z_\infty\bigr),p\bigr)-k_D(z_\infty,p)\ge \mlog 1=0\,.
$$
against Lemma~\uunoa. Thus $z_\infty\in\de D$. But then
%$$
%\limsup_{z\to z_\infty}\bigl[k_D\bigl(f(z),p\bigr)-k_D(z,p)\bigr]\ge 0\;,
%$$
%that is
$$
\liminf_{z\to z_\infty}\bigl[k_D(z,p)-k_D\bigl(f(z),p\bigr)\bigr]\le 0\;.
$$
By Proposition~\Julia\ we then have $f\bigl(E_p(z_\infty,R)\bigr)\subseteq E_p(z_\infty,R)$ for every $R>0$.
Choose $R<1$ so that $p\notin\bar{E_p(z_\infty,R)}$, and let $w\in\bar{E_p(z_\infty,R)}$ the 
point closest to~$p$ with respect to the Kobayashi distance. Since $f(w)\in\bar{E_p(z_\infty,R)}$,
it follows that $k_D\bigl(f(w),p\bigr)\ge k_D(w,p)$, which is again impossible, because $w\ne p$
and $f$ is strongly elliptic.
\qedn

\newthm
Lemma \usei:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be strongly elliptic with Wolff point $p\in D$, and let $\{z_n\}\subset D$ be a
backward orbit with Kobayashi bounded step $a=\mlog\alpha$. Then $z_n\to\sigma\in\de D$, and $\sigma$
is a boundary fixed point of $f$ with $\beta_\sigma\le\alpha$.

\pf
Let define $s_n>0$ by setting $-\mlog s_n=k_D(z_n,p)$. Without loss of generality, we can assume
that $z_0\ne p$; let $R_0=k_D(z_0,p)$, and $c=c(R_0)<1$ given by Lemma~\ucin. Arguing by induction we have
$$
k_D(z_n,p)-k_D(z_{n+1},p)\le\mlog c<0\;;
$$
in particular, $k_D(z_{n+1},p)>k_D(z_n,p)\ge R_0$ always. Hence
$$
-\mlog s_n+\mlog s_{n+1}\le\mlog c\;,
$$
that is
$$
s_{n+1}\le cs_n\;.
\neweq\equsei
$$
Therefore $s_{n+k}\le c^k s_n$ for every $n$,~$k\in\N$. So $s_n\to 0$ as~$n\to+\infty$,
that is $z_n\to\de D$, and the assertion follows from Lemma~\udue\ and  \utre.
\qedn

\newrem
We can give another proof of the convergence of a backward orbit $\{z_n\}$ with bounded Kobayashi
step~$a>0$ for strongly elliptic maps along the lines of Remark~2.1. Indeed, using \eqAS\ and
[A2,Theorem 2.3.51] we get
$$
\|z_n-z_{n+1}\|\le {C\over 1-\hat a}\sqrt{s_n}
$$
for a suitable $C>0$, where $\hat a=\tanh a$ and $-\mlog s_n=k_D(p,z_n)$. Since \equsei\
yields $s_n\le c^n s_0$, arguing as in the Remark~2.1 we see that $\{z_n\}$ is a Cauchy sequence in~$\C^d$ converging to a point~$\sigma\in\de D$.

\newthm
Lemma \usette:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be strongly elliptic with Wolff point $p\in D$. 
If $\sigma\in\de D$ is a boundary fixed point then 
$\beta_\sigma>1$.
%$$
%\alpha\ge {1\over c}>1\;.
%$$

\pf 
Indeed,  Lemma~\ucin\ yields $0<c<1$ such that
$$
\mlog\beta_\sigma=\liminf_{z\to\sigma}\bigl[k_D(z,p)-k_D\bigl(f(z),p\bigr)]\ge -\mlog c>0\;,
$$
and we are done.
\qedn

So we have proven Theorem~\OJMz.(i) and (ii); (iii) follows from the obvious fact that $p\in D$
whereas $\sigma\in\de D$. We now conclude the proof of Theorem~\OJMz\ with

\newthm
Lemma \udiecib:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain.
Let $f\in\Hol(D,D)$ be strongly elliptic, with Wolff point $p\in D$. 
Let $\{z_n\}\subset D$ be a backward orbit for~$f$ with bounded Kobayashi step converging to~$\sigma\in\de D$. Then for every $q\in D$ 
there exists $M>0$ such that $z_n\in K_{q}(\sigma,M)$ eventually.

\pf
As usual, it suffices to prove the statement for $q=p$.
Lemma \ucin\ yields $0<c<1$ such that 
$$
\liminf_{n\to\infty} [k_D(p, z_{n+1}) - k_D(p,z_n)] \ge \mlog{1\over c} >0\;,
$$
and then the assertion follows arguing as in the proof of Lemma~\udieci.
\qedn


%\newthm
%Lemma \uundici:
%Let $D\subset\subset\C^d$ be a bounded smooth strongly convex domain. Let $f\in\Hol(D,D)$ be parabolic with Wolff point $\tau\in\de D$. 
%Let $\{z_n\}\subset D$ be a backward iteration sequence for~$f$. Then $z_n\to\sigma \in \de D$ as $n\to+\infty$. 
%
%\pf
%Assume, by contradiction, that the sequence does not converge to $\de D$. Then there exists a subsequence $\{z_{n_k}\}$ converging to $w_0\in D$, that is, such that 
%$$
%k_D(w_0,z_{n_k}) \to 0 \quad \hbox{as}~k\to +\infty\;.
%$$
%Therefore
%$$
%k_D(f^{n_k}(w_0), f^{n_k}(z_{n_k})) \le k_D(w_0,z_{n_k}) \to 0 \quad \hbox{as}~k\to +\infty\;,
%$$
%which is an absurdum, because $\lim_{k\to\infty} f^{n_k}(w_0) = \tau$, and $f^{n_k}(z_{n_k}) = z_0$ for any $k$, yielding $\lim_{k\to\infty}k_D(f^{n_k}(w_0), f^{n_k}(z_{n_k})) = +\infty$.
%The assertion then follows from Lemma~\udue.
%\qedn

%\newthm
%Lemma \udodici:
%Let $D\subset\subset\C^d$ be a bounded smooth strongly convex domain. Let $f\in\Hol(D,D)$ be either hyperbolic, parabolic, or strongly elliptic, with Wolff point $\tau\in\bar{D}$. 
%Let $\{z_n\}\subset D$ be a backward iteration sequence for~$f$ with bounded Kobayashi step~$a>0$, and let $\sigma:=\lim_{n\to\infty} z_n \in \de D$. If $\sigma = \tau$, then $f$ is parabolic.
%
%\pf
%If $f$ is strongly elliptic, then $\tau \in D$, whereas $\sigma \in \de D$, and hence $\tau\ne \sigma$.
%If $f$ is hyperbolic, then by Lemma~\udieci, the sequence $\{z_n\}$ converges to $\sigma$ in a Kor\'anyi region, and we know that $z_n$ is eventually outside any horosphere in $\tau$, therefore $\tau\ne \sigma$.
%\qedn
%
%\newthm 
%Lemma \uotto:
%Let $D\subset\subset\C^d$ be a bounded smooth strongly convex domain, and fix $p\in D$. Then there exists $C>0$ such that for every $\tau\in\de D$ and every sequence $\{z_n\}\subset D$ with bounded Kobayashi step~$a>0$ we have
%$$
%\|z_n-z_{n+1}\|\le {C\over 1-\hat a}\sqrt{{1\over t_n}}\;,
%\neweq\equotto
%$$
%where $\hat a\in(0,1)$ is given by $\hat a=\tanh a$ and
%$t_n>0$ is defined by
%$$
%\mlog t_n=\lim_{w\to\tau}[k_D(w,z_n)-k_D(w,p)]\;.
%$$
%
%\pf
%By assumption, we have $k_D(z_n,z_{n+1})\le a$ for all $n\in\N$. Therefore
%Lemma~2.4 and Remark~3 of [Abate-Saracco] yields a constant $C_1>0$ such that
%$$
%\|z_n-z_{n+1}\|\le {C_1\over\sqrt{1-\hat a^2}}\sqrt{d(z_n,\de D)}\le {C_1\over 1-\hat a}\sqrt{d(z_n,\de D)}\;.
%$$
%On the other hand,
%the triangular inequality and the usual boundary estimate yield a constant $C_2>0$ such that
%$$
%\mlog t_n\le k_D(p,z_n)\le C_2-\mlog d(z_n,\de D)\;,
%$$ 
%that is
%$$
%d(z_n,\de D)\le {e^{2C_2}\over t_n}\;,
%\neweq\eqestup
%$$
%and we are done.
%\qedn
%
%\newthm 
%Lemma \unove:
%Let $D\subset\subset\C^d$ be a bounded smooth strongly convex domain, and fix $p\in D$. Then there exists $C>0$ such that for every $\tau\in\de D$ and every sequence $\{z_n\}\subset D$ with bounded Kobayashi step~$a>0$ we have
%$$
%\|z_n-z_{n+1}\|\le {C\over 1-\hat a}\sqrt{s_n}\;,
%\neweq\equnove
%$$
%where $\hat a\in(0,1)$ is given by $\hat a=\tanh a$ and
%$s_n>0$ is defined by
%$$
%-\mlog s_n=k_D(p.z_n)\;.
%$$
%
%\pf
%It works exactly as in the previous lemma.
%\qedn

\smallsect 3. Construction of backward orbits with bounded Kobayashi step

In this section we shall construct backward orbits with bounded Kobayashi
step converging to isolated boundary fixed points. To do so we need a definition
and two lemmas.

\newdef
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$.
A boundary fixed point $\sigma\in\de D$ with dilation coefficient~$\beta_\sigma$ is {\sl isolated}
if there is a neighbourhood $U\subset\C^d$ of~$\sigma$ in~$\C^d$ such that $U\cap\de D$
contains no other boundary fixed point of~$f$ with dilation coefficient at most~$\beta_\sigma$.

\newthm
Lemma \tuno:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$.
Let $\sigma\in\de D$ be a boundary fixed point of~$f$ with finite dilation coefficient $\beta_\sigma$,
and choose a complex geodesic $\phe\in\Hol(\Delta,D)$ with $\phe(1)=\sigma$. Then
$$
\lim_{t\to 1^-} k_D\bigl(\phe(t),f\bigl(\phe(t)\bigr)\bigr)={\textstyle{1\over2}}|\log\beta_\sigma|\;.
$$

\pf We shall first prove the statement when $D=\Delta$ and $\phe=\id_\Delta$. In this case
$$
k_\Delta\bigl(t,f(t)\bigr)=\mlog{1+\left|{t-f(t)\over 1-t f(t)}\right|\over 1-\left|{t-f(t)\over 1-t f(t)}\right|}\;.
$$
Now, the classical Julia-Wolff-Carath\'eodory theorem yields
$$
{1-tf(t)\over 1-t}=1+t{1-f(t)\over1-t}\to 1+\beta_1\;,\qquad
{1-tf(t)\over 1-f(t)}=1+f(t){1-t\over 1-f(t)}\to 1+{1\over\beta_1}
$$
as $t\to 1^-$; therefore
$$
{t-f(t)\over 1-t f(t)}={1-f(t)\over 1-tf(t)}-{1-t\over 1-tf(t)}\to{1\over 1+(1/\beta_1)}-{1\over 1+\beta_1}
={\beta_1-1 \over \beta_1+1}\;,
$$
and the assertion follows. 

In the general case, let $\tilde p_\phe\in\Hol(D,\Delta)$ be the left-inverse of $\phe$,
and $p_\phe=\phe\circ\tilde p_\phe$.
Put $f_\phe=p_\phe\circ f\in\Hol(D,D)$ and $\tilde f=\tilde p_\phe\circ f\circ\phe\in\Hol(\Delta,\Delta)$. First of all
$$
\eqalign{
k_D\bigl(\phe(t),f\bigl(\phe(t)\bigr)\bigr)&=k_D\bigl(\phe(t),f_\phe\bigl(\phe(t)\bigr)\bigr)+
k_D\bigl(\phe(t),f\bigl(\phe(t)\bigr)\bigr)-k_D\bigl(\phe(t),f_\phe\bigl(\phe(t)\bigr)\bigr)\cr
&=k_\Delta\bigl(t,\tilde f(t)\bigr)+k_D\bigl(\phe(t),f\bigl(\phe(t)\bigr)\bigr)-k_D\bigl(\phe(t),f_\phe\bigl(\phe(t)\bigr)\bigr)\;.\cr}
$$
Since $\sigma$ is a boundary fixed point of~$f$ it immediately follows that $1$ is a boundary
fixed point of~$\tilde f$. Furthermore, \equsf\
implies that the dilation coefficient of~$\tilde f$ at~1 is $\beta_\sigma$;
hence $k_\Delta\bigl(t,\tilde f(t)\bigr)\to{1\over2}|\log\beta_\sigma|$ as $t\to 1^-$. 
Now,
$$
\bigl|k_D\bigl(\phe(t),f\bigl(\phe(t)\bigr)\bigr)-k_D\bigl(\phe(t),f_\phe\bigl(\phe(t)\bigr)\bigr)\bigr|
\le k_D\bigl(f\bigl(\phe(t)\bigr), f_\phe\bigl(\phe(t)\bigr)\bigr)\;;
$$
so to conclude the proof it suffices to show that $k_D\bigl(f\bigl(\phe(t)\bigr), f_\phe\bigl(\phe(t)\bigr)\bigr)\to 0$ as $t\to 1^-$. 

Set $\gamma(t)=f\bigl(\phe(t)\bigr)$. By [A2, Proposition~2.7.11] it suffices to prove 
\smallskip
\item{--} that $p_\phe\circ \gamma(t)\to\sigma$ non-tangentially;
\item{--} that $\gamma(t)$ is eventually inside an
euclidean ball contained in~$D$ and tangent to~$\de D$ in~$\sigma$; 
\item{--} and that 
$$
\lim_{t\to 1^-}{\bigl\|\gamma(t)-p_\phe\bigl(\gamma(t)\bigr)\bigr\|^2\over
d\bigl(p_\phe\bigl(\gamma(t)\bigr),\de D\bigr)}=0\;.
\neweq\eqtuno
$$ 
\smallskip
Since $\phe$ is transversal to~$\de D$, to prove that $p_\phe\circ\gamma(t)\to\sigma$
non-tangentially it suffices to show that $\tilde p_\phe\circ\gamma(t)=\tilde f(t)\to 1$ non-tangentially. But the classical Julia-Wolff-Carath\'eodory theorem yields
$$
{|1-\tilde f(t)|\over 1-|\tilde f(t)|}=\left|{1-\tilde f(t)\over 1-t}\right|{1-t\over 1-|\tilde f(t)|}\to 
\beta_\sigma\cdot{1\over\beta_\sigma}=1\;,
\neweq\eqtzero
$$
and this is done.

To prove \eqtuno, we first recall that [A2, Proposition~2.7.23] yields
$$
\lim_{t\to 1^-}{\bigl\|\gamma(t)-p_\phe\bigl(\gamma(t)\bigr)\bigr\|^2\over 1-t}=0\;.
\neweq\eqtdue
$$
Furthermore, we already noticed that 
$$
\lim_{t\to 1^-}
{1-t\over 1-|\tilde f(t)|}={1\over\beta_\sigma}>0\;.
\neweq\eqttre
$$
Finally, the lower estimate [A2, Theorem~2.3.52] on the boundary behavior of the Kobayashi distance yields $c_1\in\R$ such that
$$
\mlog{1+|\tilde f(t)|\over1-|\tilde f(t)|}=k_\Delta\bigl(0,\tilde f(t)\bigr)=
k_D\bigl(\phe(0),f_\phe\bigl(\phe(t)\bigr)\bigr)\ge c_1-\mlog d\bigl(f_\phe\bigl(\phe(t)\bigr),\de D\bigr)\;,
$$
that is
$$
{1-|\tilde f(t)|\over d\bigl(f_\phe\bigl(\phe(t)\bigr),\de D\bigr)}\le 2e^{-2c_1}\;.
\neweq\eqtqua
$$
Putting together \eqtdue, \eqttre\ and \eqtqua\ we get \eqtuno.

More precisely, \eqtzero\ says that the curve $t\mapsto\tilde f(t)$ converges to~$1$ radially
(that is, tangent to the radius ending in~1); therefore the curve $p_\phe\circ\gamma$ goes to~$\sigma$ tangentially to the transversal curve $t\mapsto\phe(t)$. Furthermore, the upper estimate [A2, Theorem~2.3.51] yields $c_2\in\R$ such that
$$
\mlog{1+|\tilde f(t)|\over1-|\tilde f(t)|}\le c_2-\mlog d\bigl(f_\phe\bigl(\phe(t)\bigr),\de D\bigr)\;;
$$
hence recalling \eqttre\ and \eqtqua\ we see that $d\bigl(f_\phe\bigl(\phe(t)\bigr),\de D\bigr)$
is comparable to~$1-t$. Recalling \eqtdue\ we then obtain that $\gamma(t)$ is eventually
contained in euclidean balls internally tangent to~$\de D$ in~$\sigma$ of arbitrarily small
radius, and we are done.
\qedn

\newthm 
Lemma \tdue:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and $f\in\Hol(D,D)$.
Let $\{z_n\}\subset D$ be a sequence converging to $\sigma\in\de D$ such that 
$\limsup\limits_{n\to+\infty} k_D\bigl(z_n,f(z_n)\bigr)=\mlog\alpha<+\infty$. Then $\sigma$ is a boundary fixed
point with dilation coefficient at most~$\alpha$.

\pf
The lower estimate
[A2, Corollary~2.3.55] immediately implies that $f(z_n)\to\sigma$ as well. Fix $p\in D$; then
$$
\mlog\beta_{\sigma,p}\le\liminf_{n\to+\infty}\bigl[k_D(z_n,p)-k_D\bigl(f(z_n),p\bigr)\bigr]
\le \limsup_{n\to+\infty} k_D\bigl(z_n,f(z_n)\bigr)=\mlog\alpha\;.
$$
The assertion then follows arguing as in the proof of Lemma~\utre.
\qedn

And now we can prove the announced

\newthm
Theorem \ttre:
Let $D\subset\subset\C^d$ be a bounded strongly convex $C^2$ domain, and take $f\in\Hol(D,D)$ hyperbolic, parabolic or strongly elliptic with Wolff point $\tau\in\bar{D}$.
Let $\sigma\in\de D\setminus\{\tau\}$ be an isolated repelling boundary fixed point for~$f$ with dilation
coefficient $\beta_\sigma>1$. Then there is a backward orbit with Kobayashi step
bounded by $\mlog\beta_\sigma$
converging to~$\sigma$.

\pf
We follows closely the proof of [PC1, Lemma~1.4]. 

Let $U\subseteq\C^d$ be a small ball centered at~$\sigma$ in~$\C^d$ such that $\bar{U}\cap\bar{D}$
contains neither $\tau$ nor other boundary fixed points with dilation coefficient at most~$\beta_\sigma$, 
and put $J=\de U\cap D$. 
 
Let $\phe\in\Hol(\Delta,D)$ be a complex geodesic with 
$\phe(1)=\sigma$, and put $p=\phe(0)$. Furthermore, let $n_0\ge 0$ be such that 
$E_k=E_p(\sigma,\beta_\sigma^{-n_0-k})\subset U$ for all $k\ge 0$; set $r_k=\phe(t_k)$, where
$t_k\in(0,1)$ is such that $r_k\in\de E_k\cap\phe(\Delta)$.

For each~$k$, let $\gamma_k$ be the line segment connecting~$r_k$
and $f(r_k)$. Since $f^n(r_k)\to\tau\notin\bar{U}$, and $\bigcup_{j=0}^{n-1}f^j(\gamma_k)$ is
a path connecting $r_k$ with $f^n(r_k)$, there is a smallest integer $n_k$ such that $f^{n_k}(\gamma_k)$ intersects~$J$. Since, by Proposition~\Julia, $f(E_{k+1})\subseteq E_k$, and
the horospheres are convex, we necessarily have $n_k>k$.

Put $z_k=f^{n_k}(r_k)\in U\cap D$;
we claim that the sequence $\{z_k\}$ is relatively compact in~$D$. If not,
we can extract a subsequence $\{z_{k_j}\}$ converging to a point~$\eta\in\de D$. By 
Lemma~\tuno, $k_D\bigl(z_{k_j},f(z_{k_j})\bigr)\to\mlog\beta_\sigma$. It follows, 
by Lemma~\tdue, that $\eta$ is a boundary fixed point with dilation coefficient at most~$\beta_\sigma$;
since $\eta\in\bar{U}\cap\de D$, this contradicts the choice of~$U$.

So there is an infinite set $I_0\subseteq\N$ such that $\{z_k\}_{k\in I_0}$ converges to~$w_0\in D$. Fix $j\ge 1$, and assume that we can extract from $I_{j-1}$ an infinite set $I_j$ such that
$\{f^{n_k-j}(r_k)\}$ converges to some $w_j\in D$. Let $S=\{f^{n_k-(j+1)}(r_k)\}_{k\in I_j}$;
since 
$$
k_D\bigl(f^{n_k-(j+1)}(r_k),f^{n_k-j}(r_k)\bigr)\le k_D\bigl(r_k,f(r_k)\bigr)\to\mlog\beta_\sigma\;,
$$
the sequence $S$ is still relatively compact in~$D$, and thus we can extract from $I_j$ an
infinite set $I_{j+1}$ such that $\{f^{n_k-(j+1)}(r_k)\}_{k\in I_{j+1}}$ converges to a point $w_{j+1}\in D$. Notice that, by construction, $f(w_{j+1})=w_j$; therefore $\{w_j\}$ is a backward orbit.

Since points of the form $f^{n_k-j}(r_k)$ with $n_k>j$ are contained in~$U$, we have that
$w_j\in\bar{U}\cap D$ for all $j$. Furthermore, 
$$
k_D(w_{j+1},w_j)=\lim_{k\in I_{j+1}}k_D\bigl(f^{n_k-(j+1)}(r_k),f^{n_k-j}(r_k)\bigr)\le
\lim_{k\in I_{j+1}} k_D\bigl(r_k,f(r_k)\bigr)=\mlog\beta_\sigma\;;
$$
so we are left to prove that $w_j\to\sigma$.

Assume, by contradiction, that there is a subsequence $\{w_{j_h}\}$ converging to $q\in\bar{D}
\setminus\{\sigma\}$. If $q\in D$, then the sequence $K=\{w_{j_h}\}$ is relatively compact in~$D$;
so there is an $n>0$ such that $f^n(K)\cap U=\void$. But $K$ is a subsequence of a backward
orbit contained in~$U$, and so $f^n(K)\cap U\ne\void$ for all $n\ge 0$.

Finally, if $q\in\de D$, then, again by Lemma~\tdue, $q$ is a boundary fixed point with dilation
coefficient at most~$\beta_\sigma$; since $q\in\bar{U}$, this contradicts the choice of~$U$,
and we are done.
\qedn

\setref{PC1}
\beginsection References

\art A1 M. Abate: Horospheres and iterates of holomorphic maps! Math. Z.! 198 1988
225-238

\book A2 M. Abate: Iteration theory of holomorphic maps on taut manifolds! Mediterranean 
Press, Cosenza, 1989. See also http://www.dm.unipi.it/~abate/libri/libriric/libriric.html

\art A3 M. Abate: Iteration theory, compactly divergent sequences and commuting 
holomorphic maps! Ann. Scuola Norm. Sup. Pisa! 18 1991 167-191

\pre AS M. Abate, A. Saracco: Carleson measures and uniformly discrete sequences in strongly pseudoconvex domains! J. London Math. Soc.! 2011, doi:10.1112/jlms/jdq092

\art BP F. Bracci, G. Patrizio: Monge-Amp\`ere foliation with singularities at the boundary of strongly convex domains! Math. Ann.! 232 2005 499-522

\book JP M. Jarnicki, P. Pflug: Invariant distances and metrics in complex analysis! Walter de Gruyter \& co., Berlin, 1993

\book K S. Kobayashi: Hyperbolic complex spaces! Springer-Verlag, Berlin, 1998

\art L L. Lempert: La m\'etrique de Kobayashi et la
repr\'esentation  des domaines sur la boule! Bull. Soc. Math. France! 109 1981 427-474

\pre O O. Ostapyuk: Backward iteration in the unit ball! Preprint, arXiv:0910.5451! 2010

\art PC1 P. Poggi-Corradini: Canonical conjugations at fixed points other than the Denjoy-Wolff point! Ann. Acad. Sci. Fenn. Math.! 25 2000 487-499

\art PC2 P. Poggi-Corradini: Backward iteration sequences with bounded hyperbolic steps for analytic self-maps of the disk! Rev. Mat. Iberoamericana! 19 2003 943-970

%\newrem
%A similar argument, using the estimates
%$$
%\|z_m-z_n\|^2\le 2\sum_{j=n}^{m-1}\|z_{j+1}-z_j\|^2
%$$
%and
%$$
%\langle z_m-z_n\rangle=\sum_{j=n}^{m-1}\langle z_j+1-z_j,z_j\rangle+
%\sum_{j=n}^{m-1}\sum_{h=n}^{j-1}\langle z_{j+1}-z_j,z_h-z_{h+1}\rangle
%$$
%together with the fact, included in the proof of Lemma~2.4 in [Abate-Saracco], 
%$$
%\|z_{n+1}-z_n\|^2+|\langle z_{n+1}-z_n,z_n\rangle|\le {C\over 1-\hat a^2}d(z_n,\de D)\;,
%$$
%shows that
%$$
%\|\sigma-z_n\|^2+|\langle\sigma-z_n,z_n\rangle|\le K c^n
%$$
%for a suitable $c<1$ and $K>0$. This might be useful in proving that backward iteration sequences
%are contained in $K$-regions, because this latter statement is equivalent to finding $M>0$ such that
%$$
%\|z_n-\sigma\|^2\le M d(z_n,\de D)\quad\hbox{and}\quad |\langle z_n-\sigma,\hbox{\bf n}_\sigma\rangle|
%<M d(z_n,\de D)\;,
%$$
%where $\hbox{\bf n}_\sigma$ is the unit normal vector to~$\de D$ in~$\sigma$.  

%\Nota Another possibility is the following: \eqestup\ and \equuno\ yield $d(z_n,\de D)\le K c^n$
%for suitable $K>0$ and $c<1$. If we can show that $d(z_n,\de D)\ge k c^n$ and
%$t_nt'_n\le C$, where 
%$$
%\mlog t'_n=\lim_{w\to\sigma}[k_D(w,z_n)-k_D(w,p)]\;,
%$$
%then we are done. Unfortunately for the moment I don't know how to prove either of these.

\bye
